Solving the Discretised Neutron Diffusion Equations using Neural Networks

This paper presents a new approach which uses the tools within Artificial Intelligence (AI) software libraries as an alternative way of solving partial differential equations (PDEs) that have been discretised using standard numerical methods. In particular, we describe how to represent numerical discretisations arising from the finite volume and finite element methods by pre-determining the weights of convolutional layers within a neural network. As the weights are defined by the discretisation scheme, no training of the network is required and the solutions obtained are identical (accounting for solver tolerances) to those obtained with standard codes often written in Fortran or C++. We also explain how to implement the Jacobi method and a multigrid solver using the functions available in AI libraries. For the latter, we use a U-Net architecture which is able to represent a sawtooth multigrid method. A benefit of using AI libraries in this way is that one can exploit their power and their built-in technologies. For example, their executions are already optimised for different computer architectures, whether it be CPUs, GPUs or new-generation AI processors. In this article, we apply the proposed approach to eigenvalue problems in reactor physics where neutron transport is described by diffusion theory. For a fuel assembly benchmark, we demonstrate that the solution obtained from our new approach is the same (accounting for solver tolerances) as that obtained from the same discretisation coded in a standard way using Fortran. We then proceed to solve a reactor core benchmark using the new approach.

==> introduction_old_bits.tex <==
%This new approach also enables the relatively simple development of digital twins, using the optimisation engine and sensitivities embedded in AI software. The digital twins can be used to optimise systems, form error measures, assimilate data and quantify uncertainty in a relatively straightforward manner with this approach. This enables the major deficiency (formation of an error estimate) in current modelling approaches for safety critical systems in nuclear engineering to be addressed.

Due to new hardware technologies, increases in computing power and developments in AI software, the benefits of combining AI techniques with traditional numerical methods for solving governing equations of dynamical systems are becoming apparent. Cerebras have just released a new ‘AI computer’ called CS-2~\citep{cerebras} which has about 1~million cores on a single chip with vastly increased computational speed, yet which requires much less energy than GPUs or CPUs, making it ideal hardware for researchers to run computationally demanding problems in an energy-efficient manner. If the potential of combining the new AI computers and AI software with traditional numerical methods can be harnessed, one can expect a revolution in computational physics across disciplines and a `must have' next-generation technology. Based on the latest techniques in AI software, this paper reports the first steps of a potentially revolutionary approach to the discretisation and solution of differential equations and applies it to the multi-group diffusion equation for neutron transport. Our approach implements conventional discretisations using AI software with the aim of simplifying the code development and exploiting the very substantial developments already made in AI technology, for example, code abstraction and platform agnosticism. This simplification could greatly increase the number of researchers able to become more involved in the development of current models (each code is often limited to a handful of expert developers), speeding up its implementation and its parallel scalability. 


Recent techniques utilising the many software technologies of AI for predicting physical phenomena described through some underlying differential equation are extensive, and only a small sample of works can be mentioned here. Perhaps one of the most significant works developed in this field is that of \cite{RAISSI2019686} that paved the way for the use of deep neural networks (DNN) to form solutions to both forward and inverse problems of systems described by PDEs. Using the backpropagation technique within the DNN, one can automatically differentiate a network's output,  the solution to the PDE, with respect to its input and the spatial-temporal dimension, to form residuals of the equations that then feed into its training. Applied to a class of problems from fluids, quantum mechanics, and reaction-diffusion systems, the approach has been adopted to fields stretching across fluid dynamics, heat transfer, materials, solid mechanics and radiative transport \cite{MISHRA2021107705}. A particularly powerful aspect of using such approaches are they inherently designed to assimilate observational data and so have been used to form solutions to many physical systems when data is available. Early works include using data from passive dyes,  smoke, or vapour to extract solutions to the Navier-Stokes equations~\cite{cai_2021,PINNS_Raissi}. Others include the use of PINNs for analysing subsurface transport \cite{HE2020103610}, and for other fluid problems where the mix of computational (LES-CFD) and experimental data (particle image velocimetry) were used to identify missing quantities in turbulent flows \cite{Saldern}. AI technologies are evermore being used in digital twins, whereby they are employed to form fast surrogate models (reduced order models (ROMs)) of systems for real-time analysis. One of the particular advantages of the approach is its non-intrusive implementation, meaning there is no need to solve high-fidelity models in order to form surrogate models. One way to achieve this is to combine DNNs with more traditional ROM technologies, such as Proper Orthogonal Decomposition (POD)~\cite{Lumley1967}, Greedy POD,  and empirical interpolation methods (EIM)~\cite{xiao2014non}, where the latter provides compression of solution space to a small number of fundamental modes, whilst in the former the DNN are trained to predict models coefficients. Other approaches are to use DNNs with shrinking and expanding layers of neurons to perform the compression of the solution space through auto-encoders~\cite{phillips2021}. These methods have been further adapted for large-scale heterogeneous systems, for example through domain decomposition approaches, and applied to fields covering nuclear engineering and multi-phase flows~\cite{heaney2022ai}.

The approach described in this article is a new, and alternative, way of harnessing AI technologies for forming solutions of governing PDEs. Here it is proposed to perform the computations that form the solution from standard discretisation techniques through convolutional layers. Ultimately these result in the identical solutions of the discretised models, but the advantage here is that performing all operations through the AI allows optimal code efficiency on all architectures whilst enabling the latest developments in methods such as sensitivities~\cite{cervi2022sensitivity}, uncertainty quantification~\cite{kabir2018neural} and data assimilation~\cite{amendola2020data}, thanks to the neural network architecture.
The research proposed here, therefore, has the potential to cause a shift in the way numerical models are developed and used. The beneficiaries will be wide-ranging, including any researchers or organisations requiring PDE models and associated AI-Physics models. The ability to rely on high-level libraries that can seamlessly integrate AI tools with PDE models, will both reduce development time with increased performance portability and increase parallel scalability. 
Whilst adaptable to general PDE operators and fields of physics, this article has focused on the field of nuclear reactor physics and solves the neutron transport eigenvalue problem, as described through diffusion theory. Furthermore, whilst underlying discretisation methods can be arbitrary, our demonstration focuses on the use of CNN to replicate the solution process when using the control volume method together with a NN-based multigrid algorithm for fast solution convergence.


In the field of nuclear energy, AI is becoming  popular and has been applied to inverse problems for accident analysis \cite{CUI2022109257}, NN for power control of PWRs \cite{XIAO2022108946}, and PINNS have been developed for point kinetics simulations \cite{SCHIASSI2022108833}. In \cite{FOAD2022109017} they have been used as ROMs and combined PCA with DNNs for transient analysis, auto-encoders developed for eigenvalue problems \cite{phillips2021}, in \cite{QIN2020107785} DNNs were used for neutron cross-section generation, and in \cite{NSE_DTR} a digital twin for neutron diffusion calculations was proposed. PINNS have also been developed across subdomains of problems and used for solving non-smooth heterogeneous neutron diffusion problems \cite{WANG2022109234}.

%\section{intro-old-hold}






%Due to new hardware technologies, increases in computing power and developments in AI software, the benefits of combining AI techniques with traditional numerical methods for solving governing equations of dynamical systems are becoming apparent. For example, Cerebras have just released a new ‘AI computer’ called CS-2~\citep{cerebras} which has about 1~million cores on a single chip with vastly increased computational speed, yet which requires much less energy than GPUs or CPUs, making it a tantalising prospect for researchers wishing to run demanding computations in an energy efficient manner. If the potential of combining the new AI computers and AI software with traditional numerical methods can be harnessed, one can expect a revolution in computational physics across disciplines and a ‘must have’ next generation technology. Based on the latest techniques in AI software, this paper reports first steps of a potentially revolutionary approach to the discretisation and solution of differential equations and applying these to solve the multi-energy group diffusion equation for neutron transport. Our approach implements conventional discretisations using AI software with the aim of simplifying the software development and building on the very substantial developments already made in AI software. This simplification would greatly increase the number of developers capable of developing current model (each code often limited to a handful of expert developers), speeding up the implementation of developments and their parallel scalability. This new approach also enables relatively simple development of digital twins, using the optimisation engine and sensitivities embedded in AI software. The digital twins can be used to optimise systems, form error measures, assimilate data and quantify uncertainty [7] in a relatively straightforward manner with this approach. This enables the major deficiency (formation of an error estimate) in current modelling approaches for safety critical systems in nuclear engineering to be addressed.  





%Deep learning has become increasingly popular for scientific computing applications, including AI-Physics models, and is now a common workload for supercomputers, using significant resources. The common ways to parallelise deep learning across multiple GPUs/CPUs are data parallelism and model parallelism. However, the details of the implementation greatly affect the scaling efficiency. There are several competing implementations of data-parallel deep learning that are currently used in production on distributed systems. For work on solving differential equations that are able to exploit parallelisation of AI using Domain Decomposition, see [8,9]. Also, existing approaches for solving differential equations involve re-implementation of the dynamic cores using OPS or OP2 [10] for structured and unstructured meshes to ensure interoperability between CPUs and GPUs. 


%Programming Partial Differential Equations (PDEs) using AI software is potentially revolutionary in computational physics particly because it enables interoperability between GPUs, CPUs and AI computers and exploitation of AI community software. Energy shortfalls and climate change mean that the use of energy efficient computers are particularly important and we thus aim for a demonstration of the approach on an AI computer (Cerebras, see ***). 

%The key advantages of programming PDE numerical solution methods using AI software include: (a) Solvers: Linear, non-linear multigrid methods and gradient based non-linear solutions (e.g. Newton Raphson) can be applied relatively easily implemented using convolutional autoencoders in AI software. AI models can also be readily used as preconditions in CFD matrix equation solvers.  (b) By leveraging existing AI software libraries one can realise new features in modelling without writing large quantities of code e.g. for use of mixed arithmetic precision (speed of model); coupling different physics. (c) Using AI software would make model development more accessible than programming existing CFD models - similar to other AI applications. (d) The code generated by programming in AI software would be automatically optimised and be interoperable between computer architectures: CPU, GPU and AI computers - including exascale computers. (e) Long term model/code sustainability as code is based on long standing, community supported, AI software. 

%The research proposed here has the potential to cause a shift in the way numerical models are developed and used. The beneficiaries will be wide-ranging, including any researchers or organisations requiring PDE models and associated AI-Physics models. The ability to rely on high-level libraries that can seamlessly integrate AI tools with PDE models, will both reduce development time with increased performance portability and parallel scalability. 

The sections of this paper is organised as follows. Section \ref{methods} presents the theory for the use of NN in solving the neutron diffusion equations together with its multigrid solver for the control volume discretisation. Section \ref{results} presents the 3 numerical examples using the NN solver to resolve reactor physics eigenvalue problems, and comparisons are drawn against a standard control volume method. Finally, section \ref{conclusion} completes the paper with a conclusion of its findings. 
